Sculpting Subspaces: Constrained Full Fine-Tuning in LLMs for Continual Learning

Continual learning in large language models (LLMs) is prone to catastrophic forgetting, where adapting to new tasks significantly degrades performance on previously learned ones. Existing methods typically rely on low-rank, parameter-efficient updates that limit the model's expressivity and introduce additional parameters per task, leading to scalability issues. To address these limitations, we propose a novel continual full fine-tuning approach leveraging adaptive singular value decomposition (SVD). Our method dynamically identifies task-specific low-rank parameter subspaces and constrains updates to be orthogonal to critical directions associated with prior tasks, thus effectively minimizing interference without additional parameter overhead or storing previous task gradients. We evaluate our approach extensively on standard continual learning benchmarks using both encoder-decoder (T5-Large) and decoder-only (LLaMA-2 7B) models, spanning diverse tasks including classification, generation, and reasoning. Empirically, our method achieves state-of-the-art results, up to 7% higher average accuracy than recent baselines like O-LoRA, and notably maintains the model's general linguistic capabilities, instruction-following accuracy, and safety throughout the continual learning process by reducing forgetting to near-negligible levels. Our adaptive SVD framework effectively balances model plasticity and knowledge retention, providing a practical, theoretically grounded, and computationally scalable solution for continual learning scenarios in large language models.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> past_versions/conclusion_v1.tex <==
\section{Conclusion}
\label{sec:conclusion}
Large language models (LLMs) have become foundational to numerous real-world applications, but their true potential is unlocked only through \emph{post-training customization}—the process of adapting models to continuously evolving data, tasks, and user demands. In enterprise deployments, this translates into the critical need for \emph{continual learning}: updating models with new information without compromising previously acquired capabilities. However, standard approaches to post-training, such as LoRA-based fine-tuning or maintaining separate models per task, suffer from fundamental inefficiencies—either due to constrained expressivity or unsustainable parameter growth.

This work presents a scalable, expressive, and theoretically grounded solution to this challenge. We introduce an adaptive continual fine-tuning method that operates in the full parameter space but constrains updates to low-rank subspaces orthogonal to previously learned knowledge. Our method delivers strong empirical results across a wide spectrum of settings. On the \textbf{standard 5-task continual learning benchmark}, our approach achieves \textbf{79.6\%} accuracy with LLaMA-2 7B and outperforms O-LoRA by over 3 points which is the current SOTA. On the more challenging \textbf{15-task sequence}, it maintains \textbf{71.3\%} accuracy with T5-Large—outperforming all parameter-efficient and replay-based baselines. On the \textbf{TRACE benchmark}, using the \textbf{LLaMA-2 7B-Chat} model, our method achieves the highest average accuracy (\textbf{48.4\%}) among all methods not requiring multi-task access or task-specific models. Importantly,our method also preserves general ability, instruction-following, and safety, making it especially suitable for real-world deployments.


==> past_versions/experimental_v1.tex <==
\section{Experiment Results}
In this section, we present an extensive evaluation of our adaptive SVD-based continual learning approach against state-of-the-art baselines, with particular emphasis on comparisons to Orthogonal Low-Rank Adaptation (O-LoRA)~\cite{wang2024olora}. We describe the experimental setup, benchmarks, baselines, and the empirical results highlighting the effectiveness and advantages of our proposed method.

\subsection{Experimental Setup}

We evaluate our method on widely-used continual learning benchmarks for language models, following the experimental settings established by prior state-of-the-art works, specifically the O-LoRA framework~\cite{wang2024olora}.

\textbf{Standard Continual Learning Benchmark (5 tasks)}: This benchmark consists of five text classification datasets introduced by Zhang et al. (2015):
\begin{itemize}
\item \textbf{AG News}: News classification into four categories (World, Sports, Business, Sci/Tech).
\item \textbf{Amazon Reviews}: Sentiment analysis on product reviews (very negative/negative/neutral/positive/very positive).
\item \textbf{Yelp Reviews}: Sentiment analysis on restaurant reviews (very negative/negative/neutral/positive/very positive).
\item \textbf{DBpedia}: Topic classification based on Wikipedia articles.
\item \textbf{Yahoo Answers}: Topic classification into ten categories.
\end{itemize}

\textbf{Extended Continual Learning Benchmark (15 tasks)}: To evaluate performance in more challenging scenarios involving longer task sequences, we follow Razdaibiedina et al. (2023) by including:
\begin{itemize}
\item All 5 tasks from the standard benchmark.
\item 4 tasks from the GLUE benchmark (MNLI, QQP, RTE, SST2).
\item 5 tasks from the SuperGLUE benchmark (WiC, CB, COPA, MultiRC, BoolQ).
\item IMDB movie reviews dataset for sentiment classification.
\end{itemize}

For each task, we train on 14,000 randomly selected samples and validate using 7,600 samples, evenly distributed across classes. We evaluate our approach on two model architectures: the encoder-decoder T5-Large and the decoder-only LLaMA-2 7B.

\subsection{Baselines}

We benchmark our approach against a comprehensive set of continual learning methods, spanning fine-tuning, regularization, replay, adapter-based, and prompt-based techniques. Notably, O-LoRA~\cite{wang2024olora} provides a strong baseline and represents the current state of the art. In particular, we include:

\begin{itemize}

\item \textbf{SeqFT}~\cite{de2019episodic}: Sequential full-model fine-tuning without additional constraints or replay mechanisms.
\item \textbf{SeqLoRA}: Sequential fine-tuning using fixed-size LoRA adapters.
\item \textbf{IncLoRA}: A variant of LoRA where new low-rank adapters are incrementally added and trained as tasks progress.
\item \textbf{Replay}: Experience replay by maintaining a buffer of samples from previous tasks.
\item \textbf{EWC (Elastic Weight Consolidation)}~\cite{kirkpatrick2017overcoming}: Regularization-based approach penalizing important parameter updates.
\item \textbf{LwF (Learning without Forgetting)}~\cite{li2017learning}: Maintains shared representations to mitigate forgetting.
\item \textbf{L2P}~\cite{wang2022learning}: Learns a pool of prompts and dynamically selects relevant prompts for each input during inference.
\item \textbf{LFPT5}~\cite{qin2021lfpt5}: Trains a continuous soft prompt that jointly learns the tasks and generates replay data.
\item \textbf{O-LoRA}~\cite{wang2024olora}: Maintains a history of all previously trained LoRA adapters and enforces orthogonality when learning new ones; all adapters are then merged into a single adapter at inference time.
\item \textbf{ProgPrompt}~\cite{razdaibiedina2023progressive}: Maintains separate soft prompts for each task, growing the prompt set over time. This implicitly stores task-specific information and requires task IDs for inference, making it less scalable.
\item \textbf{PerTaskFT}: Trains a separate model for each task. While effective, it assumes access to all task-specific data and models during training and inference, which is impractical in real-world deployments.
\item \textbf{MTL (Multi-Task Learning)}: Trains a single model jointly on all tasks simultaneously, representing an upper bound on performance but relaxing the continual learning constraint of task-wise sequential training.
\end{itemize}

Unlike methods that grow parameters with the number of tasks (e.g., IncLoRA, O-LoRA, ProgPrompt, PerTaskFT) or rely on strong assumptions about task separation (e.g., PerTaskFT, MTL), our approach introduces no additional parameters—even as the number of tasks grows—and does not assume prior knowledge of task identity or access to all data at once. This makes it particularly well-suited for scalable and deployable continual learning in enterprise settings.


\subsection{Results}

We summarize the results in Table~\ref{tab:results_summary}. We report the \textbf{Average Accuracy (AA)}, a widely-used metric in continual learning. It measures the average test accuracy across all tasks \textit{after} training on the final task. Formally, if the model has been trained on $T$ tasks and $A_{T,j}$ denotes the test accuracy on task $j$ after learning all $T$ tasks, the average accuracy is defined as:
\begin{equation}
\text{AA} = \frac{1}{T} \sum_{j=1}^{T} A_{T,j}
\end{equation}

Following the evaluation protocol used in O-LoRA ~\cite{wang2024olora}, all results are averaged over 3 runs with different permutations of the task sequence. Our adaptive SVD-based method consistently achieves higher performance compared to all baselines, including the strong O-LoRA approach.


\begin{table}[h]
\centering
\caption{Comparison of Average Accuracy (\%) across standard continual learning benchmarks}
\label{tab:results_summary}
\begin{tabular}{lcc}
\toprule
\textbf{Method} & \textbf{T5-Large (5 tasks)} & \textbf{T5-Large (15 tasks)} \\
\midrule
SeqFT & 28.5 & 7.4 \\
SeqLoRA & 43.7 & 1.6 \\
IncLoRA & 66.4 & 61.2 \\
Replay & 57.8 & 54.2 \\
EWC & 48.7 & 45.1 \\
LwF & 52.3 & 46.9 \\
L2P & 60.7 & 56.1 \\
LFPT5 & 72.7 & 69.2 \\
O-LoRA & 75.8 & 69.6 \\
\textbf{Ours (Adaptive SVD)} & \textbf{75.9} & \textbf{71.3} \\
\midrule
ProgPrompt & 75.1 & 77.9 \\
PerTaskFT & 70.0 & 78.1 \\
MTL (Upper Bound) & 80.0 & 76.5 \\
\bottomrule
\end{tabular}
\end{table}

For the LLaMA-2 7B model on the 5-task benchmark, we achieve an average accuracy of \textbf{79.6\%}, surpassing the previous state-of-the-art O-LoRA, which achieved 76.1\%. We also run ablation studies to understand the importance of two core components in our method: (1) accurate estimation of effective rank, and (2) constraining updates to remain within the low-rank subspace. Results are shown in Appendix~\ref{appendix:ablations}.

\subsection{Parameter Efficiency Analysis}

A critical distinction between our approach and O-LoRA lies in parameter efficiency. O-LoRA requires additional task-specific low-rank parameter matrices ($\Delta W$) for each task, increasing parameter storage linearly with the number of tasks. Specifically, O-LoRA stores matrices of dimensions $n \times r$ per task and needs to maintain all previous matrices for future inference or additional training.

In contrast, our method requires \textit{no additional parameters}, regardless of the number of tasks learned, ensuring constant memory and computational costs as tasks accumulate. This offers a significant scalability advantage over O-LoRA, particularly important as continual learning scenarios become more complex and long-term.

\subsection{Evaluation on TRACE Continual Learning Benchmark}

To further assess the robustness of our proposed adaptive SVD method in realistic continual learning settings, we evaluate it on the TRACE benchmark~\cite{wang2023trace}, a recently introduced suite specifically designed to test the limits of aligned large language models under sequential task learning. TRACE addresses the shortcomings of earlier continual learning benchmarks by incorporating more diverse, challenging, and instruction-tuned tasks that better reflect real-world use cases.

The benchmark comprises eight sequential tasks that span multiple capabilities: domain-specific understanding, multilingual reasoning, code completion, and mathematical reasoning. Specifically, the tasks include ScienceQA, FOMC, and MeetingBank for domain-specific knowledge; C-STANCE and 20Minuten for multilingual understanding; Py150 for code completion; and two arithmetic reasoning tasks from NumGLUE. Each dataset introduces new task formats and data distributions, which collectively challenge the model’s ability to learn continually while retaining prior knowledge.

We use the LLaMA-2-7B-Chat model as the backbone and compare our approach against a range of strong baselines used in TRACE: (1) sequential full-parameter fine-tuning (SeqFT), (2) LoRA-based sequential fine-tuning (LoRASeqFT), (3) replay-based fine-tuning (Replay), and (4) in-context learning (ICL) using task demonstrations as prompts. Following the TRACE protocol, we evaluate performance using two main metrics: Overall Performance (OP), which measures the average accuracy across all tasks after sequential training, and Backward Transfer (BWT), which captures the extent of forgetting by comparing current performance on previous tasks to the performance at the time they were first learned.

We use the LLaMA-2-7B-Chat model as the backbone and compare our approach against a range of strong baselines used in TRACE, including: (1) sequential full-parameter fine-tuning (SeqFT), (2) LoRA-based sequential fine-tuning (LoRASeqFT), (3) replay-based fine-tuning (Replay), (4) in-context learning (ICL) using task demonstrations as prompts, (5) Orthogonal LoRA (O-LoRA), (6) Progressive Prompts (PP), (7) Single-task fine-tuning (PerTaskFT), and (8) Multi-task learning (MT). Following the TRACE evaluation protocol, we report performance using two key metrics: \textit{Average Accuracy (AA)}, which measures the average performance across all tasks after the final task has been learned as before, and \textit{Backward Transfer (BWT)}, which quantifies how much the model forgets earlier tasks during continual learning. BWT is calculated as:
\begin{equation}
\text{BWT}_t = \frac{1}{t} \sum_{i=1}^{t-1} \left(R^D_{t,i} - R^D_{i,i}\right)
\end{equation}
where $R^D_{t,i}$ denotes the model’s accuracy on task $i$ after learning task $t$, and $R^D_{i,i}$ denotes the accuracy on task $i$ immediately after it was learned. A positive BWT indicates improved retention, while negative values indicate forgetting.

As shown in Table~\ref{tab:trace_results}, our method significantly outperforms SeqFT, LoRASeqFT, and Replay in both OP and BWT. In particular, while standard SeqFT suffers from strong negative BWT due to catastrophic forgetting, our approach maintains positive backward transfer and strong performance across all tasks, demonstrating its ability to retain prior knowledge while effectively learning new information.

\begin{table}[h]
\centering
\caption{Performance on the TRACE continual learning benchmark using LLaMA-2-7B-Chat. Higher OP and BWT indicate better retention and adaptation.}
\label{tab:trace_results}
\begin{tabular}{lcc}
\toprule
\textbf{Method} & \textbf{OP (\%)} & \textbf{BWT (\%)} \\
\midrule
ICL & 39.5 & -- \\
ICL + Replay & 41.1 & -- \\
SeqFT & 23.0 & -8.3 \\
O-LoRA & 41.3 & 6.2 \\
\textbf{Ours (Adaptive SVD)} & \textbf{48.4} & \textbf{7.1} \\
\midrule
ProgPrompt & 46.2 & 2.3 \\
PerTaskFT & 57.6 & -- \\
MT & 52.3 & -- \\
\bottomrule
\end{tabular}
\end{table}

In addition to continual learning performance, we assess whether the model retains its core capabilities after sequential training along three key axes: \textit{general language understanding and reasoning ability}, \textit{instruction-following ability}, and \textit{safety}. This evaluation setup follows the TRACE benchmark~\cite{wang2023trace}, which emphasizes the importance of preserving aligned behaviors in LLMs during continual learning. General ability is measured using a diverse suite of benchmarks, including MMLU for factual knowledge, GSM8K for arithmetic reasoning, BBH for multi-step general reasoning, TyDiQA for multilingual question answering, PIQA for commonsense reasoning, and BoolQ for reading comprehension. Instruction-following is evaluated using the Self-Instruct dataset, which contains a wide variety of user-facing prompts across domains such as productivity, creative writing, and programming, and the LIMA dataset, which includes carefully curated human-authored queries from online Q\&A forums. To assess safety, we use the CoNa dataset, which consists of prompts designed to elicit potentially harmful or toxic outputs; responses are evaluated based on whether the model maintains safe and non-offensive behavior. Preserving performance across these three axes is essential for real-world deployments, where degradation in any one area can undermine user trust and system reliability.

For each of these categories, we compute the average delta in performance before and after continual learning, representing the net degradation or improvement in model behavior following~\cite{wang2023trace}. For example, the General Ability Delta is computed as:
\begin{equation}
\Delta R^G_t = \frac{1}{M} \sum_{i=1}^{M} (R^G_{t,i} - R^G_{0,i}),
\end{equation}
where $R^G_{t,i}$ is the performance on the $i$-th general task after training on task $t$, and $R^G_{0,i}$ is the baseline performance on the $i$-th task before any continual training, and $M$ is the total number of general evaluation tasks. Analogous formulas are used for Instruction Following Delta ($\Delta R^I_t$) and Safety Delta ($\Delta R^S_t$).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.80\textwidth]{images/general_ability.pdf}
    \caption{Comparison of general ability scores across six diverse evaluation tasks between the base LLaMA-2-7B-Chat model and our adaptive SVD-based continual learner.}
    \label{fig:general_ability_plot}
\end{figure}

As shown in Figure~\ref{fig:general_ability_plot}, our approach maintains or improves performance across most general ability benchmarks relative to the base instruction-tuned model, particularly in multilingual QA, comprehension, and commonsense reasoning. The observed degradation in mathematical and general reasoning tasks (GSM, BBH) is a common effect of task-specific fine-tuning and can be mitigated by combining our method with reasoning-augmented approaches like Reasoning-augmented Continual Learning (RCL)~\cite{wang2023trace}, as we discuss in the following paragraph. Similarly, as shown in Table~\ref{tab:trace_help_safety_breakdown}, our method exhibits lower loss rates and higher or comparable win/tie rates across both instruction-following and safety.

\begin{table}[h]
\centering
\caption{Win / Tie / Lose breakdown (\%) for instruction-following and safety evaluations against the LLaMA-2-7B-Chat base model.}
\label{tab:trace_help_safety_breakdown}
\begin{tabular}{lccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Instruction (Helpfulness)}} & \multicolumn{3}{c}{\textbf{Safety}} \\
 & Win & Tie & Lose & Win & Tie & Lose \\
\midrule
Replay & 10 & 18 & 72 & 0 & 88 & 12 \\
LoRASeqFT & 3 & 4 & 94 & 0 & 86 & 14 \\
SeqFT & 14 & 34 & 53 & 0 & 98 & 2 \\
\textbf{Ours (Adaptive SVD)} & \textbf{24} & \textbf{56} & \textbf{20} & \textbf{18} & \textbf{78} & \textbf{4} \\
\bottomrule
\end{tabular}
\end{table}

This highlights the advantage of constraining updates to low-rank subspaces orthogonal to previously learned tasks—enabling knowledge retention across both task-specific and foundational capabilities. Our method not only achieves strong continual learning performance on complex multi-domain tasks, but also preserves the general reasoning, safety, and instruction-following capabilities essential for deployment in practical settings. Our method can also be effectively combined with complementary techniques like RCL~\cite{wang2023trace} and replay buffers to further enhance learning and mitigate forgetting. RCL, introduced in the TRACE benchmark~\cite{wang2023trace}, augments training data with reasoning paths that guide the model toward clearer task-specific understanding and better task transfer, helping preserve the model’s inherent reasoning abilities during sequential learning. Separately, replay buffers enable periodic rehearsal of previously seen tasks, reinforcing old knowledge while new tasks are learned. Notably, these strategies are highly compatible with our approach—RCL enhances task clarity and generalization, while replay buffers strengthen memory retention, and together with our method, they offer a promising direction for building more robust and adaptable continual learners.


==> past_versions/introduction_v1.tex <==
\section{Introduction}
\label{sec:intro}
Large language models (LLMs) have revolutionized natural language understanding and generation, demonstrating remarkable proficiency in various tasks, including classification, complex reasoning, and generation \citep{brown2020language, chowdhery2022palm, touvron2023llama}. Despite these capabilities, constantly adapting these models to new tasks without compromising previously acquired knowledge, known as continual learning, remains an open challenge \citep{kirkpatrick2017overcoming, zenke2017continual}. Catastrophic forgetting, defined by substantial deterioration in performance on prior tasks after training on subsequent tasks, poses a significant obstacle, particularly given the complexity and scale inherent to modern LLMs \citep{mccloskey1989catastrophic, french1999catastrophic, luo2025empirical}.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.20\textwidth]{images/method_illustration.pdf}
%     \caption{High-level overview of our adaptive SVD-based continual learning method. We decompose weight matrices via SVD, identify low-rank subspaces orthogonal to previous tasks' gradients, and apply projected gradient descent to avoid interference with prior knowledge. High-rank subspace aligns with old task data; learning happens in low-rank directions.}
%     \label{fig:method_overview}
% \end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.05\textwidth, trim={110 20 110 20}, clip]{images/method_illustration.pdf}
    \caption{High-level overview of our adaptive SVD-based continual learning method. We decompose weight matrices via SVD, identify low-rank subspaces orthogonal to previous tasks' gradients, and apply projected gradient descent to avoid interference with prior knowledge. High-rank subspace aligns with old task data; learning happens in low-rank directions.}
    \label{fig:method_overview}
\end{figure}

Existing approaches to continual learning primarily include parameter-efficient fine-tuning methods, such as adapters and Low-Rank Adaptation (LoRA), and strategies utilizing parameter isolation or orthogonality constraints \citep{houlsby2019parameter, hu2022lora, wang2024olora, liang2024inflora, serra2018overcoming}. Although effective in mitigating forgetting, these approaches limit the model's expressive capacity, require additional parameters per task, and face difficulties in capturing complex task-specific nuances \citep{wang2024olora, liang2024inflora}.

Alternatively, sequential full-model fine-tuning, where all model parameters are updated without constraints, fully leverages the expressive capacity of LLMs. However, this approach remains notoriously susceptible to catastrophic forgetting due to conflicting updates between tasks \citep{luo2025empirical}. Thus, a fundamental challenge emerges: 
\begin{center}
\emph{How can we leverage the flexibility of full-model updates without sacrificing knowledge retention between the tasks?}    
\end{center}


We address this gap by proposing a novel continual full fine-tuning approach that dynamically identifies low-rank subspaces within model parameter matrices using adaptive Singular Value Decomposition (SVD). Our method restricts parameter updates to adaptive low-rank subspaces specifically chosen to be orthogonal to previously learned task representations, ensuring minimal interference and substantially reducing catastrophic forgetting. This strategy provides several advantages:

\begin{itemize}
    \item It fully exploits the expressive capacity of LLMs by updating the entire parameter set in carefully selected subspaces.
    \item It does not require additional parameters or storage of previous task data or gradients.
    \item It dynamically adapts subspace selection per task based on theoretical insights from geometric and spectral analyses, minimizing interference.
\end{itemize}

The theoretical grounding of our adaptive subspace selection draws from geometric and spectral analyses, guiding updates into directions with minimal interference. We empirically validate our approach on established continual learning benchmarks using multiple language models of different scales up to 10 billion parameters, comparing comprehensively against state-of-the-art continual fine-tuning methods. Our results demonstrate that our method achieves superior performance, effectively mitigating catastrophic forgetting while leveraging the representational power of the entire model. A visual overview of our method is shown in Figure~\ref{fig:method_overview}.

The remainder of this paper is structured as follows. Section~\ref{sec:related_work} reviews relevant continual learning methods. Section~\ref{sec:methodology} introduces our adaptive subspace-based fine-tuning method with theoretical justifications. Section~\ref{sec:experimental_setup} describes the benchmarks and evaluation metrics. The results are presented in Section~\ref{sec:results}, and detailed discussions and analyses are provided in Section~\ref{sec:discussion}. Finally, Section~\ref{sec:conclusion} summarizes our contributions and outlines future research directions.


==> past_versions/limitations_v1.tex <==
\textbf{Limitations and Future Directions.} While the proposed method is simple and effective, it relies on accurate estimation of the effective rank of a matrix to determine which singular directions must remain fixed. In our exploration, we experimented with several strategies—including allocating a fixed number of singular vectors per task, applying entropy-based thresholds, leveraging random matrix theory, and adopting a normalized input–output similarity metric, among others. However, as shown in our ablations (Appendix~\ref{appendix:ablations}), when this estimation is inaccurate, performance noticeably degrades. Developing principled theoretical tools to bound the effective rank remains an important direction for future work. Second, our method, in its simplest and effective form, operates under a pre-allocated budget per task by freezing a portion of high singular vectors. When the number of tasks is unknown, however, determining how much capacity to reserve for each task becomes challenging. Lastly, while our method updates all matrices in the model—including all attention and MLP projections—it remains an open question whether similar performance can be achieved by fine-tuning only a subset of matrices. Prior work on parameter-efficient fine-tuning has shown that adapting only the query and value matrices can yield competitive results. Exploring selective fine-tuning strategies may yield further improvements in efficiency without sacrificing performance.


==> past_versions/methodology_v1.tex <==
\section{Methodology}
\label{sec:methodology}

In this section, we detail our proposed adaptive Singular Value Decomposition (SVD)-based continual learning approach, which dynamically identifies low-rank subspaces orthogonal to previously learned task representations to minimize catastrophic forgetting. We provide both intuitive explanations and theoretical foundations to justify our method's effectiveness.

\subsection{Problem Formulation}
\label{subsec:problem_formulation}

Given a sequence of tasks $\{D_1, D_2, \ldots, D_T\}$, where each task $D_t$ consists of data samples $\{(x_i^t, y_i^t)\}_{i=1}^{n_t}$, the objective of continual learning is to sequentially learn these tasks while maintaining performance on all previously learned tasks. We focus on large language models with parameters $\theta$ that are updated during the learning process.

For each weight matrix $\mathbf{W} \in \mathbb{R}^{d_O \times d_I}$ in the network, we aim to find parameter updates that effectively learn the current task while minimizing interference with previous tasks. This can be formulated as:

\begin{equation}
\min_{\Delta \mathbf{W}} \mathcal{L}_{t}(\theta + \Delta \theta) \quad \text{s.t.} \quad \Delta \mathbf{W} \perp \mathcal{M}_{t-1}
\end{equation}

where $\mathcal{L}_{t}$ is the loss function for task $t$, $\Delta \theta$ represents the parameter updates, and $\mathcal{M}_{t-1}$ represents the subspace of parameters important for previous tasks.

\subsection{Adaptive SVD-Based Fine-Tuning}
\label{subsec:adaptive_svd}

Our method leverages the full parameter space of language models while strategically minimizing interference between sequential tasks. For each layer's weight matrix, we first perform SVD:

\begin{equation}
    \mathbf{W} = \mathbf{U}\Sigma\mathbf{V}^{\top},
\end{equation}

where $\mathbf{U} \in \mathbb{R}^{d_O \times d_O}$ and $\mathbf{V} \in \mathbb{R}^{d_I \times d_I}$ contain the left and right singular vectors, respectively, and $\Sigma \in \mathbb{R}^{d_O \times d_I}$ is the diagonal matrix of singular values $\sigma_1 \geq \sigma_2 \geq \ldots \geq \sigma_{\min(d_O, d_I)} \geq 0$.

We then dynamically partition the singular vectors into two complementary subspaces:
\begin{itemize}
    \item High-rank subspace $(\mathbf{U}_h, \mathbf{V}_h)$ associated with larger singular values, encoding critical knowledge from previous tasks
    \item Low-rank subspace $(\mathbf{U}_l, \mathbf{V}_l)$ associated with smaller singular values, representing directions less critical to prior tasks
\end{itemize}

Parameter updates for new tasks are constrained to this low-rank subspace:
\begin{equation}
    \Delta\mathbf{W} = \mathbf{U}_l \Delta\Sigma_l \mathbf{V}_l^{\top},
\end{equation}

This approach ensures that updates remain orthogonal to the high-rank subspace that encodes previous task knowledge, effectively minimizing forgetting while enabling the model to adapt to new information.

\subsection{Adaptive Rank Determination}
\label{subsec:rank_determination}

The critical question becomes: how do we determine the appropriate rank for partitioning the singular vector space? We utilize an adaptive approach inspired by theoretical insights from random matrix theory \citep{marchenko1967distribution} and recent findings in SVD-based compression \citep{li2025adasvd}.

For each layer $l$, we compute a retention ratio $r_l$ based on the layer's importance:

\begin{equation}
r_l = \text{mrr} + I_n(\mathbf{W}_l) \cdot (\text{trr} - \text{mrr})
\end{equation}

where $\text{mrr}$ is the minimum retention ratio, $\text{trr}$ is the target retention ratio, and $I_n(\mathbf{W}_l)$ is the normalized importance of layer $l$. The importance is measured based on the layer's influence on model outputs, determined through gradient magnitudes during initial training.

This approach ensures that more critical layers (typically found in earlier and final transformer blocks) retain more of their singular vectors in the high-rank subspace, while less critical intermediate layers can accommodate more significant changes.

\subsection{Projected Gradient Descent for Orthogonal Updates}
\label{subsec:projected_gradient}

To enforce orthogonality with the high-rank subspace during training, we employ projected gradient descent. For each gradient update, we project the gradient onto the orthogonal complement of the high-rank subspace $\mathcal{M}_{t-1}$:

\begin{equation}
\nabla \mathbf{W}_{\text{proj}} = \nabla \mathbf{W} - \mathbf{U}_h\mathbf{U}_h^T\nabla \mathbf{W}\mathbf{V}_h\mathbf{V}_h^T
\end{equation}

This projection operation ensures that gradient updates do not interfere with directions encoding previous task knowledge, effectively minimizing catastrophic forgetting while enabling efficient learning of new tasks.

\subsection{Theoretical Analysis}
\label{subsec:theoretical_analysis}

We now present a theoretical guarantee that learning in low-rank subspaces orthogonal to previous task representations minimizes forgetting.

\begin{theorem}
Let $\mathcal{M}_{t-1}$ be the subspace spanned by the high-rank singular vectors of weight matrices for tasks $1, \ldots, t-1$, and let $\mathcal{M}_{t-1}^{\perp}$ be its orthogonal complement. If parameter updates $\Delta \mathbf{W}$ for task $t$ lie in a low-rank subspace of $\mathcal{M}_{t-1}^{\perp}$, then the interference with previous tasks is minimized to first order.
\end{theorem}

\begin{proof}
Consider the loss $\mathcal{L}_{<t}$ on previous tasks after updating the parameters for task $t$. Let $\Delta \mathbf{W}$ be the parameter update for task $t$. The change in loss for previous tasks can be approximated (to first order) as:

\begin{equation}
\Delta \mathcal{L}_{<t} \approx \text{Tr}(\nabla_{\mathbf{W}} \mathcal{L}_{<t} \cdot \Delta \mathbf{W}^T)
\end{equation}

The gradient $\nabla_{\mathbf{W}} \mathcal{L}_{<t}$ represents the direction in parameter space that affects the loss on previous tasks. By the properties of SVD and the nature of neural network training, this gradient predominantly lies in the subspace $\mathcal{M}_{t-1}$ formed by the high-rank singular vectors.

If $\Delta \mathbf{W} \in \mathcal{M}_{t-1}^{\perp}$ (i.e., $\Delta \mathbf{W} \perp \mathcal{M}_{t-1}$), then:

\begin{equation}
\text{Tr}(\nabla_{\mathbf{W}} \mathcal{L}_{<t} \cdot \Delta \mathbf{W}^T) = 0
\end{equation}

This is because the trace of the product of orthogonal matrices is zero. Thus, parameter updates that lie in $\mathcal{M}_{t-1}^{\perp}$ do not increase the loss on previous tasks to first order.

Furthermore, by restricting $\Delta \mathbf{W}$ to a low-rank subspace of $\mathcal{M}_{t-1}^{\perp}$, we ensure that only the most effective directions for the current task are used, maximizing learning efficiency while maintaining orthogonality with previous task representations.
\end{proof}

This theorem extends concepts from InfLoRA \citep{liang2024inflora} to the adaptive SVD-based setting, providing a theoretical foundation for why our constrained low-rank updates are effective for continual learning.

\subsection{Exploration of Alternative Rank Approximation Methods}
\label{subsec:alternative_methods}

Prior to developing our adaptive SVD approach, we extensively explored alternative effective rank approximation methods from recent literature, including LASER \citep{sharma2023laser} and SPECTRUM fine-tuning \citep{panigrahi2023spectrum}. 

LASER employs a fixed rank-reduction strategy across selected layers, while SPECTRUM uses noise-level thresholds derived from random matrix theory to identify ranks. Our empirical evaluations revealed that these approaches, while effective for single-task learning, faced limitations in continual learning scenarios:

\begin{itemize}
    \item Fixed-rank approaches (including LASER) failed to account for the varying importance of different layers, leading to suboptimal trade-offs between plasticity and stability
    \item SPECTRUM's thresholds, while theoretically motivated, proved unstable during sequential task learning when tasks exhibited substantially different distributions
    \item Neither approach explicitly enforced orthogonality with previous task subspaces, a critical requirement for minimizing forgetting
\end{itemize}

These limitations motivated our development of the adaptive rank determination method that dynamically adjusts subspace partitioning based on layer importance and explicitly enforces orthogonality constraints.

\subsection{Validation of Low-Rank Subspace Assumptions}
\label{subsec:assumption_validation}

A key assumption of our approach is that lower singular vectors (corresponding to smaller singular values) can be repurposed without significantly impacting performance on previous tasks. To validate this assumption, we conducted preliminary experiments systematically pruning increasing proportions of lower singular vectors from pre-trained models.

Our results consistently showed that pruning up to x\% of the lowest singular vectors resulted in negligible performance degradation on held-out validation sets. This empirical finding aligns with theoretical work suggesting that neural networks contain substantial parameter redundancy \citep{frankle2018lottery}, and supports our approach of adaptively repurposing low-rank subspaces during continual learning.



==> past_versions/theory_V1.tex <==
\subsection{Theoretical Analysis: Tighter Forgetting Bounds via Adaptive SVD}
\label{appendix:theorem_tight_bounds}

We now formally derive a hierarchy of catastrophic forgetting bounds that rigorously demonstrate the advantage of our adaptive rank selection approach compared to both naive full fine-tuning and uniform low-rank projection methods.

\begin{lemma}[Second-Order Approximation of Catastrophic Forgetting]
\label{lemma:second_order_approx}
Consider a model with parameters \(\theta^{(k)}\) after training on task \(k\), and subsequent parameters \(\theta^{(k+1)} = \theta^{(k)} + \Delta\theta\) after learning task \(k+1\). Assuming \(\nabla L_k(\theta^{(k)}) \approx 0\) (i.e., task \(k\)'s loss is near-optimal at \(\theta^{(k)}\)), the catastrophic forgetting on task \(k\) can be approximated by:
\begin{equation}
\Delta L_k \triangleq L_k(\theta^{(k+1)}) - L_k(\theta^{(k)})
\approx
\frac{1}{2}\Delta\theta^\top H_k \Delta\theta,
\end{equation}
where \(H_k=\nabla^2 L_k(\theta^{(k)})\) is the Hessian of the loss function at \(\theta^{(k)}\).
\end{lemma}

\begin{proof}
Expanding \(L_k\) at \(\theta^{(k+1)} = \theta^{(k)} + \Delta\theta\) via Taylor's theorem:
\begin{equation}
L_k(\theta^{(k+1)}) 
=
L_k(\theta^{(k)}) 
+ 
\underbrace{\nabla L_k(\theta^{(k)})^\top \Delta\theta}_{\approx 0}
+ 
\frac{1}{2}\Delta\theta^\top H_k \Delta\theta + O(\|\Delta\theta\|^3).
\end{equation}

Since \(\theta^{(k)}\) represents a (local) optimum for task \(k\), we have \(\nabla L_k(\theta^{(k)}) \approx \mathbf{0}\). With the first-order term vanishing due to optimality, the performance degradation is dominated by the quadratic term, yielding our result.
\end{proof}

\begin{lemma}[Block-Diagonal Approximation of the Hessian]
\label{lemma:block_diagonal}
The Hessian matrix \(H_k\) can be approximated as a block-diagonal matrix with respect to layers:
\begin{equation}
H_k \approx \begin{bmatrix}
H_k^{(1)} & 0 & \cdots & 0 \\
0 & H_k^{(2)} & \cdots & 0 \\
\vdots & \vdots & \ddots & \vdots \\
0 & 0 & \cdots & H_k^{(L)}
\end{bmatrix}
\end{equation}
where each \(H_k^{(\ell)}\) represents the layer-wise Hessian for layer \(\ell\). Under this approximation:
\begin{equation}
\Delta\theta^\top H_k \Delta\theta \approx \sum_{\ell=1}^{L} vec(\Delta W^{(\ell)})^\top H_k^{(\ell)} vec(\Delta W^{(\ell)})
\end{equation}
\end{lemma}

\begin{proof}
This approximation is justified by empirical evidence showing that inter-layer Hessian interactions are typically small compared to intra-layer interactions \citep{ghorbani2019investigation, pascanu2013difficulty}. Given the layer-wise decomposition of the parameter vector \(\theta = [vec(W^{(1)})^\top, vec(W^{(2)})^\top, \ldots, vec(W^{(L)})^\top]^\top\), the quadratic form decomposes as shown.
\end{proof}

\begin{lemma}[Relationship Between Layer Importance and Curvature]
\label{lemma:importance_curvature}
The layer importance measure \(I^{(\ell)}\), defined as:
\begin{equation}
I^{(\ell)} = \frac{1}{N}\sum_{i=1}^{N} \text{cosine\_similarity}(X_i^{(\ell)}, Y_i^{(\ell)})
\end{equation}
where \(X_i^{(\ell)}\) are layer inputs and \(Y_i^{(\ell)} = W^{(\ell)}X_i^{(\ell)}\) are layer outputs, positively correlates with the spectral properties of the layer-wise Hessian \(H_k^{(\ell)}\).
\end{lemma}

\begin{proof}
Layers with high importance scores (high similarity between inputs and outputs) tend to preserve activation patterns rather than significantly transform them. These layers typically serve as information conduits in the network, maintaining critical features learned for task \(k\). 

Empirically, these high-importance layers exhibit higher sensitivity to parameter perturbations. When a layer primarily passes information forward with minimal transformation (high \(I^{(\ell)}\)), perturbations to its parameters directly interfere with this information flow, causing large changes in the loss function. Mathematically, this translates to larger eigenvalues in \(H_k^{(\ell)}\), indicating steeper curvature.

Conversely, layers with lower \(I^{(\ell)}\) values significantly transform their inputs, suggesting these layers are more adaptable. Perturbations to these layers' parameters cause smaller changes in the loss landscape, resulting in smaller eigenvalues in \(H_k^{(\ell)}\).

This relationship has been verified empirically in multiple studies \citep{sharma2023truth, li2025adasvdadaptivesingularvalue}, consistently showing a positive correlation between measures of layer importance and the magnitude of Hessian eigenvalues.
\end{proof}

We can now present our main theorem on the hierarchy of forgetting bounds across different fine-tuning strategies.

\begin{theorem}[Hierarchy of Forgetting Bounds]
\label{thm:forgetting_bounds_hierarchy}
Assuming equal parameter update magnitudes \(\|\Delta\theta\|^2 = c\) across different fine-tuning strategies, the forgetting bounds satisfy:
\begin{equation}
\text{Adaptive SVD} < \text{Fixed-Rank} < \text{Full Fine-tuning}
\end{equation}
Specifically:
\begin{align}
\text{Full Fine-tuning:} & \quad \Delta L_k \leq \frac{1}{2}\lambda_{\max}(H_k) \cdot c \\
\text{Fixed-rank:} & \quad \Delta L_k \leq \frac{1}{2}\max_\ell\{\lambda_{r+1}^{(\ell)}\} \cdot c \\
\text{Adaptive (Ours):} & \quad \Delta L_k \leq \frac{1}{2}\max_\ell\{\lambda_{r(\ell)+1}^{(\ell)}\} \cdot c
\end{align}
where \(r(\ell) = \text{mrr} + I^{(\ell)}(\text{trr} - \text{mrr})\) is our adaptive rank allocation based on layer importance.

Moreover, under the condition that layer importance \(I^{(\ell)}\) positively correlates with Hessian curvature (Lemma \ref{lemma:importance_curvature}), we have:
\begin{equation}
\max_\ell\{\lambda_{r(\ell)+1}^{(\ell)}\} < \max_\ell\{\lambda_{r+1}^{(\ell)}\} \leq \lambda_{\max}(H_k)
\end{equation}
ensuring our adaptive approach provides strictly tighter forgetting bounds.
\end{theorem}

\begin{proof}
We establish the hierarchy of bounds by proving each inequality separately.

\textbf{Part 1:} \(\max_\ell\{\lambda_{r+1}^{(\ell)}\} \leq \lambda_{\max}(H_k)\).

By the block-diagonal approximation (Lemma \ref{lemma:block_diagonal}), \(\lambda_{\max}(H_k) = \max_\ell\{\lambda_1^{(\ell)}\}\). Since \(\lambda_{r+1}^{(\ell)} \leq \lambda_1^{(\ell)}\) for all \(\ell\) by the ordering of eigenvalues, we have:
\begin{equation}
\max_\ell\{\lambda_{r+1}^{(\ell)}\} \leq \max_\ell\{\lambda_1^{(\ell)}\} = \lambda_{\max}(H_k)
\end{equation}

\textbf{Part 2:} \(\max_\ell\{\lambda_{r(\ell)+1}^{(\ell)}\} < \max_\ell\{\lambda_{r+1}^{(\ell)}\}\).

Let \(\ell^* = \operatorname{arg\hspace{0.7mm}max}_\ell \lambda_{r+1}^{(\ell)}\) be the layer with the largest post-projection eigenvalue in the fixed-rank approach. By Lemma \ref{lemma:importance_curvature}, this layer typically has high curvature, and thus high importance \(I^{(\ell^*)}\).

Under our adaptive allocation strategy, this high-importance layer receives a larger rank allocation (\(r(\ell^*) > r\)), ensuring:
\begin{equation}
\lambda_{r(\ell^*)+1}^{(\ell^*)} < \lambda_{r+1}^{(\ell^*)} = \max_\ell\{\lambda_{r+1}^{(\ell)}\}
\end{equation}

For any other layer \(\ell \neq \ell^*\), we have:
\begin{equation}
\lambda_{r(\ell)+1}^{(\ell)} < \lambda_{r+1}^{(\ell^*)} = \max_\ell\{\lambda_{r+1}^{(\ell)}\}
\end{equation}
either because \(r(\ell) > r\) (for other high-importance layers) or because \(\lambda_{r+1}^{(\ell)} < \lambda_{r+1}^{(\ell^*)}\) (for low-importance layers, even if \(r(\ell) < r\)).

Therefore, \(\max_\ell\{\lambda_{r(\ell)+1}^{(\ell)}\} < \max_\ell\{\lambda_{r+1}^{(\ell)}\}\), establishing the strict improvement of our adaptive approach over fixed-rank projection.

Combining Parts 1 and 2 completes the proof of the bound hierarchy.
\end{proof}

\begin{corollary}[Forgetting Reduction with Adaptive SVD]
\label{cor:forgetting_reduction}
Under the equal parameter update magnitude assumption, our adaptive SVD-based approach achieves strictly less catastrophic forgetting than both fixed-rank projection and full fine-tuning methods.
\end{corollary}

\begin{proof}
Follows directly from Theorem \ref{thm:forgetting_bounds_hierarchy} and the established bound hierarchy:
\begin{equation}
\Delta L_k^{\text{Adaptive}} < \Delta L_k^{\text{Fixed-rank}} < \Delta L_k^{\text{Full}}
\end{equation}
\end{proof}

This theoretical analysis provides the formal justification for our adaptive SVD approach, demonstrating why it consistently outperforms both full fine-tuning and uniform low-rank projection strategies in mitigating catastrophic forgetting. The result confirms that by intelligently allocating rank budgets based on layer importance, which correlates with curvature in the loss landscape, we achieve a strictly tighter bound on forgetting while maintaining update flexibility. This establishes a principled foundation for adaptive parameter-efficient fine-tuning in continual learning scenarios.

This theoretical result provides the formal justification for our adaptive SVD approach, demonstrating why it consistently outperforms both full fine-tuning and uniform low-rank projection strategies in mitigating catastrophic forgetting. Our analysis bridges the gap between empirical observations and theoretical understanding, establishing a principled foundation for adaptive parameter-efficient fine-tuning in continual learning scenarios.

